Imaging radial velocity planets with SPHERE

We present observations with the planet finder SPHERE of a selected sample of the most promising radial velocity (RV) companions for high-contrast imaging. Using a Monte Carlo simulation to explore all the possible inclinations of the orbit of wide RV companions, we identified the systems with companions that could potentially be detected with SPHERE. We found the most favorable RV systems to observe are : HD\,142, GJ\,676, HD\,39091, HIP\,70849, and HD\,30177 and carried out observations of these systems during SPHERE Guaranteed Time Observing (GTO). To reduce the intensity of the starlight and reveal faint companions, we used Principle Component Analysis (PCA) algorithms alongside angular and spectral differential imaging. We injected synthetic planets with known flux to evaluate the self-subtraction caused by our data reduction and to determine the 5$\sigma$ contrast in the J band $vs$ separation for our reduced images. We estimated the upper limit on detectable companion mass around the selected stars from the contrast plot obtained from our data reduction. Although our observations enabled contrasts larger than 15 mag at a few tenths of arcsec from the host stars, we detected no planets. However, we were able to set upper mass limits around the stars using AMES-COND evolutionary models. We can exclude the presence of companions more massive than 25-28 \MJup around these stars, confirming the substellar nature of these RV companions.

==> ref_letter.tex <==
- We modified the paragraph according to the referee's suggestion;
- Indeed, important references were missing and we thank the referee to point that out. We added them in the main text;
- We modified the paragraph according to the referee's suggestion;
- We corrected the inconsistency in the text, the minimum separation chosen was 0.1 arcsec, slightly smaller than the dimension of the mask, to be conservative;
- We removed the redundant phrase;
- We changed the Figures accordingly;
- We changed the Figure 6 accordingly;
- The fact that some targets are binaries is just a coincidence, we selected all the targets observable with SPHERE, and since we ended up with a very limited sample (5 targets), and the binarity was not a problem for the observations, we did not exclude any of them; 
- It is probable that since we used uniform linear distributions to generate the periods of the binary, we are biased towards long period results. We added a phrase in the main text with this caveat;
- We changed the Figure 8 accordingly;
- We added in the main text the contrast needed to detect GJ 676 Ac in the assumption that it is coplanar to the other planet b;
- We added the separations in the main text;
- We splitted the Conclusions in multiple paragraphs;
- The formulas and contents of the Appendix have also been presented in Zurlo's PhD thesis, which has been read by two external referees, N. Thatte and A. Sozzetti, who carefully checked the contents of the thesis. Also, the co-authors read and commented the manuscript. 

